Improving Personalisation in Valence and Arousal Prediction using Data Augmentation

In the field of emotion recognition and Human-Machine Interaction (HMI), personalised approaches have exhibited their efficacy in capturing individual-specific characteristics and enhancing affective prediction accuracy. However, personalisation techniques often face the challenge of limited data for target individuals. This paper presents our work on an enhanced personalisation strategy, that leverages data augmentation to develop tailored models for continuous valence and arousal prediction. Our proposed approach, Distance Weighting Augmentation (DWA), employs a weighting-based augmentation method that expands a target individual's dataset, leveraging distance metrics to identify similar samples at the segment-level. Experimental results on the MuSe-Personalisation 2023 Challenge dataset demonstrate that our method significantly improves the performance of features sets which have low baseline performance, on the test set. This improvement in poor-performing features comes without sacrificing performance on high-performing features. In particular, our method achieves a maximum combined testing CCC of 0.78, compared to the reported baseline score of 0.76 (reproduced at 0.72). It also achieved a peak arousal and valence scores of 0.81 and 0.76, compared to reproduced baseline scores of 0.76 and 0.67 respectively. Through this work, we make significant contributions to the advancement of personalised affective computing models, enhancing the practicality and adaptability of data-level personalisation in real world contexts.

==> MuSeChallenge/ReviewsMuseChallenge.tex <==
----------------------- REVIEW 1 ---------------------
SUBMISSION: 4
TITLE: Distance Weighting Augmentation for Valence and Arousal Prediction Under Data Constraints
AUTHORS: Munachiso Nwadike, Jialin Li, Ananta Manoranjan and Hanan Salam

----------- Technical Correctness -----------
SCORE: 3 (Minor issues but credible results)
----------- Comments on technical correctness if severely flawed or significant flaws. -----------
The overall pipeline and adherence to the challenge protocol look fine. However, as shall be mentioned later in more detail, one of the distance measures used / proposed, namely the centroid DP, is not a distance but a similarity measure. Thus experiments with this measure should be either removed or reproduced after corrections.
----------- Clarity of Presentation -----------
SCORE: 3 (Clear enough, could benefit from some revision)
----------- Comments on clarity of presentation if difficult to read or follow. -----------
Overall it can be understood clearly. Minor suggestions for typos / corrections
- page 1: define the open form of BPM % OK
- page 1: 'to enhance the accuracy of machine learning sentiment analysis.' -> Why do you think this task is sentiment analysis? Arousal and valence are emotion primitives. % ok 
- page 3: 'In this paper we refer to the 55 training and testing individuals as D_G...' -> You mean 'In this paper, we refer to the 55 training and development individuals ... ' ? %ok 
- page 4: 'The BCF' -> 'the BCF' % OK 
- page 5, Table 2: For better comparison, it will be handy to add the corresponding baseline performances to Table 2.
- page 5: 'the valence score increases from 0.84 to 0.70'-> 'the valence score increases from 0.70 to 0.84'
- page 5: 'the massive improvement in performance'-> 'the dramatic improvement in performance' % OK 
- page 6, Table 3: 'Basline Devel' -> 'Baseline Devel'
----------- Overall evaluation -----------
SCORE: 1 (weak accept)
----- TEXT:
The paper proposes a simple (weighted data augmentation) method to select windows (understood as audio/visual descriptors from the rest of the paper) that are the most similar to the test instances and conduct an individualization (a second stage) fine-tuning after a first stage global fine-tuning of pre-trained networks with the all available training data.

Strengths:
- The proposed method is simple and effective, as shown by the results on the challenge data.

Weaknesses and suggestions for further improvement:
- The method proposed has incremental novelty. It mentions weighting, which gives an impression of a weighted loss function to be employed with respect to the window similarity. However, the weights end up being binary, namely a selection of the frames is then applied. While the actual use of more nuanced weights in [0, 1] rather than in {0, 1} has the potential to further improve the performance if combined with the weighing of the loss function.

- The centroid DP (as shown in the algorithm and in eq. 2, is not a distance but a similarity measure. Thus, if you have used this as a distance measure with minimum n, then you have trained on the most dissimilar instances. This may explain the inconsistent performance/behavior when using this measure. The reviewer suggests converting the similarity into a distance measure and renewing experiments. One approach would be to negating the dot product or subtracting it from a constant C. C can be determined theoretically, if we have prior information about the scale/normalization of the features (e.g., if the features are standardized and have dimensionality of d, simply we can set C = d due to summation of expectation of z^2=1). Otherwise, one needs to get an empirical maximum to set C. Another alternative is using cosine distance on the centroids, as in the case of the other measure that applies this distance per sample. % OK 



----------------------- REVIEW 2 ---------------------
SUBMISSION: 4
TITLE: Distance Weighting Augmentation for Valence and Arousal Prediction Under Data Constraints
AUTHORS: Munachiso Nwadike, Jialin Li, Ananta Manoranjan and Hanan Salam

----------- Technical Correctness -----------
SCORE: 2 (Significant flaws that may call results into question)
----------- Comments on technical correctness if severely flawed or significant flaws. -----------
Section 2.1: "...DWA begins by constructing an augmentation pool AP from DG, which comprises all samples (i.e., windows) S, from all individuals in the training and development sets..." 
=> In my opinion, there are lacking information w.r.t. the composition of the augmentation pool. Precisely, it is not clear for me in the description of the distance weighting augmentation approach if "all samples from all individuals in the training and development set" refers to the 55 participants or if also the partially available snippets of the 14 test participants are also included? In my opinion, the augmentation pool should only consist of the 55 participants as only the partially available test data of one person (the one on which the model is personalised to) should be used for its personalisation. If all snippets of all 14 test participants are part of the augmentation pool, then it is maybe not a complete fair comparision. In my opinion, this needs to be outlined in detail in the methodology section (Section 2).
----------- Clarity of Presentation -----------
SCORE: 3 (Clear enough, could benefit from some revision)
----------- Comments on clarity of presentation if difficult to read or follow. -----------
Overall it is well written, but there are minor issues. E.g.: 
- Section 4.1: "...On the development set, the valence score increases from 0.84 to 0.70..." => Should probably be "...increases from 0.70 to 0.84..."
- In the paper it is often mentioned that particular methods work "significantly" better. Have the authors performed any kind of significance test?
----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----- TEXT:
Overall, I think the paper proposes an interesting approach. However, in my opinion there are several minor issues which are stated above. In addition, the distance weighting augmentation should be described in more detail in the methodology section.

Overall recommendation: weak reject



----------------------- REVIEW 3 ---------------------
SUBMISSION: 4
TITLE: Distance Weighting Augmentation for Valence and Arousal Prediction Under Data Constraints
AUTHORS: Munachiso Nwadike, Jialin Li, Ananta Manoranjan and Hanan Salam

----------- Technical Correctness -----------
SCORE: 2 (Significant flaws that may call results into question)
----------- Comments on technical correctness if severely flawed or significant flaws. -----------
1) The authors reflect correctly on the fact that different feature sets capture different characteristics. Hence, for FaceNet features, the method can be expected to augment individual datasets with data from people that look similar to the test subject. The egemaps features, in contrast, directly capture variations in prosody. Given that different features capture different aspects, I wonder why the authors have only experimented with two of them.

    2) As the authors also indicate, simply averaging (or summing up cosine similarities) over a window of 10s, i.e. 20 steps leads to loss of sequential information. It is unclear, if the averaging operation leaves one with actually meaningful data. No ablation study or the like is provided with a smaller window. 

    3) Related to 2), I wonder if the similarities between average values of many high-dimensional features are meaningful. There is no analysis on the distribution of similarity values. E.g., it could be that similarities do not differ much and thus carry little information 

    4) I am not convinced of the method’s performance. If I understood correctly, one configuration (augmented FaceNet + non-augmented egemaps) outperformed the baseline test result by a slight margin (~.78 compared to ~.76).
----------- Clarity of Presentation -----------
SCORE: 3 (Clear enough, could benefit from some revision)
----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----- TEXT:
The paper is well-structured, proposes a novel method based on augmenting data for each individual and reports on a plethora of experiments. However, I have some doubts about the method, cf. above.


Some detailed comments on the presentation:
- "constitutes form" -> "constitutes a form" (p.1)
- "The MuSe-Personalisation baseline paper" (p.1): citation missing 

- Fig. 1 would benefit a lot from explicitly including the augmentation approach

- Algorithm 1: 
    - l.1-6 can be shortened, AP is just the unioin over all samples of all individuals 
    - computing the distance metrics can be shortened by giving the metric as a parameter. These formulas look a bit confusing in the algorithm and they are already given in the text 

- The three distance metrics should not be subsubsections 

- "solo conversations" (p.3) sounds like a contradiction

- Structure of Table 1 is unclear: what do "Training", "Devel" and "Test" refer to, respectively? Also, the checkmark indicating label availability should be noted in the caption.

- Including the baseline in Table 2 would be highly beneficial. The Combined baseline score is never mentioned.

- p.5 "valence score increases from 0.84 to 0.70"


==> draft.tex <==
Recently, there has been a shift in affective computing research from controlled laboratory environments to more realistic natural settings, allowing for the analysis of a wider range of subtle, continuous emotional and health states in real-world scenarios. This has led to the formulation of continuous ER as a dimensional problem, using a valence-arousal space to represent complex human emotions. Valence measures the pleasantness of emotions, ranging from negative (such as sadness) to positive (like happiness), while arousal spans from passive (like sleepiness) to active (such as high excitement) [6]. Recognizing these nuanced emotional states is valuable in applications like assessing driver fatigue, estimating levels of depression or pain in healthcare, and evaluating customer engagement in marketing. Given the increasing demand for continuous ER in real-world contexts, this paper focuses on dimensional ER in the valence-arousal space.

%\textcolor{red}{TODO Experiments: }
% \begin{enumerate}
%     \item we need to have experiments with and without data augmentation. This is what would show that the proposed approach is improving the results. 
%     \item Run models for all the features and their combinations with the 3 distance metrics.
%     \item Choosing empirical values for n is not methodologically correct: implement hyperparameter optimization for n, you can use Grid Search, or any other optimization method.
%     \item Summarize the reviewers comments regarding the experiments and do them. 
%     \item Compare the approach to state-of-the art approaches.  This means we need to create a table that compares our best performance to the state of the art approaches, namely, baseline and the other participants results. 
%     \item Table 3: I am not sure why the results in this table are not on the test set. What is baseline Devel? 
%     \item I am not sure I understand well n: is it the number of samples (window segments) you add to the training set to augment it? so n = 1 means that you augmented the dataset by only 1 sample? if this is the case, then there is a huge problem. Adding only one sample is insignificant.
% \end{enumerate}
